SVG-IR: Spatially-Varying Gaussian Splatting for Inverse Rendering

Reconstructing 3D assets from images, known as inverse rendering (IR), remains a challenging task due to its ill-posed nature. 3D Gaussian Splatting (3DGS) has demonstrated impressive capabilities for novel view synthesis (NVS) tasks. Methods apply it to relighting by separating radiance into BRDF parameters and lighting, yet produce inferior relighting quality with artifacts and unnatural indirect illumination due to the limited capability of each Gaussian, which has constant material parameters and normal, alongside the absence of physical constraints for indirect lighting. In this paper, we present a novel framework called Spatially-vayring Gaussian Inverse Rendering (SVG-IR), aimed at enhancing both NVS and relighting quality. To this end, we propose a new representation-Spatially-varying Gaussian (SVG)-that allows per-Gaussian spatially varying parameters. This enhanced representation is complemented by a SVG splatting scheme akin to vertex/fragment shading in traditional graphics pipelines. Furthermore, we integrate a physically-based indirect lighting model, enabling more realistic relighting. The proposed SVG-IR framework significantly improves rendering quality, outperforming state-of-the-art NeRF-based methods by 2.5 dB in peak signal-to-noise ratio (PSNR) and surpassing existing Gaussian-based techniques by 3.5 dB in relighting tasks, all while maintaining a real-time rendering speed.

==> tex/temp.tex <==
\begin{equation}
    L_i(\mu_s, \omega_i) = 
    \sum^n_{i=0}{c_l\alpha_l\prod_{p=1}^{l-1}(1-\alpha_p)}+ L_{\mathrm{dir}}V,
\end{equation}
where $c_l$ and $\alpha_l$ is the radiance field color and  transparency computed as ~\ref{eq:gsfilter} by $o_l$, $V$ is the visibility to the ambient light. The $T_{\mathrm{threshold}}$ is set as 0.2.

Therefore, we still need to model the indirect illumination in reflectance field. Utilizing the index buffer $I_i$ obtained from the previous ray tracing step, we can easily identify the first Gaussian visible from each Gaussian in the hemisphere direction, thereby achieving equivalent one-bounce ray tracing to obtain indirect radiance from reflectance field $L_{i}^{\mathrm{ind}'}$ as
\begin{equation}
    L_{i,j}^{\mathrm{ind}'}(x, \omega_i^j) = \sum_{k=1}^{m} \frac{f(x',\omega_{i}^{k},-\omega_{i}^{j})L_{I_i(j)}^{\mathrm{dir}}(\omega_{i}^{k},x')(\omega_{i}^{k},n)}{p(\omega_{i}^{k})},
\end{equation}
where $L_{i,j}^{\mathrm{ind}'}$ is the indrect radiance from reflectance field from the $i$-th Gaussian in the $j$-th direction. It is calculated by the Monte Carlo integration of the shading results in each $k$-th direction on the second hit Gaussian, where $p(\omega_{i}^{k})$ is the probability density function in the direction $\omega_{i}^{k}$. 
This allows us to obtain more accurate indirect illumination under the new light source, derived from the reflectance field.
